A Human-Centered Dynamic Scheduling Architecture for Collaborative Application

In collaborative robotic applications, human and robot have to work together during a whole shift for executing a sequence of jobs. The performance of the human robot team can be enhanced by scheduling the right tasks to the human and the robot. The scheduling should consider the task execution constraints, the variability in the task execution by the human, and the job quality of the human. Therefore, it is necessary to dynamically schedule the assigned tasks. In this paper, we propose a two-layered architecture for task allocation and scheduling in a collaborative cell. Job quality is explicitly considered during the allocation of the tasks and over a sequence of jobs. The tasks are dynamically scheduled based on the real time monitoring of the human's activities. The effectiveness of the proposed architecture is experimentally validated.

==> sections/6_dynamic_scheduling.tex <==
% \begin{itemize}
%     \item Description of the dynamic Scheduler and its behavior:
%     \begin{itemize}
%         \item 1. nominal behavior (no unexpected event and human nominal execution time)
%         \item 2. the human is slow (dynamic scheduler anticipate tasks for the robot and or reassign some tasks improving job quality)
%         \item 3. robot can not execute a task (communication and assign the task with maximum priority)
%         \item 4. human decides to swap a task (communication and assign the task with maximum priority)
%     \end{itemize}
%     \item Pseudocode of the algorithm
%     \item Adaptation of the initial weights based on the human monitoring
% \end{itemize}
Starting from the output of the Task Assignment, the goal of the Dynamic Scheduler is to adapt online the two nominal schedules $S_H$ and $S_R$ taking into account the uncertainty of the human behavior. When two humans collaborate, their natural synergy allows to reach high performance of the team. If one human gets slower the other might compensate by speeding up. Furthermore, more complex unexpected difficulties are handled by communication. The most expert member of the team can exploit his knowledge to reorganize the work or decide to perform some part of the work. On the other side, when in trouble, the less experienced member of the team asks the expert member for some help. The dynamic scheduler aims at reproducing this kind of behavior in human-robot collaboration in order to create an effective and natural cooperation.
	
This is achieved exploiting two different strategies. Firstly, the human operator is monitored in real time when performing the task in order to estimate the real execution time and, if necessary, to reschedule the future activities of the robot, avoiding useless waiting time. Secondly, the communication between the human and the robot is enabled, allowing the two agents to take decisions about their activities through the scheduler. In particular, the robot delegates a task it cannot momentarily execute to the human. The human, instead, can decide to execute the task that the robot is performing (because, e.g., from its experience, it feels that the robot is not executing the task in a proper way) or he will have to execute (because, e.g., he wants to speed up the workflow). Moreover, the human can decide to re-assign some of his tasks to the robot. The dynamic scheduler is implemented according to the pseudo-code reported in Alg.~\ref{alg:dynamicscheduler}.
	
\begin{algorithm}
    \caption{DynamicScheduler()}
    \label{alg:dynamicscheduler}
    \begin{algorithmic}[1]
    	\State \textbf{Require:} $S_H$,$S_R$\label{algl:dsrequire}
    	\State $End_R ,End_H \leftarrow false$ \label{algl:dsinitializeends}
    	\State $l \leftarrow 1$ \label{algl:dsinitializelevel}
    	\If{$S_R(l) \ne \emptyset$ \label{algl:dsinitializetasksstart}} $T_R \leftarrow S_R(l,1)$\EndIf
    	\If{$S_H(l) \ne \emptyset$} $T_H \leftarrow S_H(l,1)$
    	\EndIf \label{algl:dsinitializetasksend}
		\While{$l \leq L$} \label{algl:dswhilelevels}
    	\While{$(T_R\ne\emptyset$ \textbf{and} $T_H\ne\emptyset)$  \label{algl:dswhiletasks}}  	\If{$T_R=\emptyset$ \label{algl:dsrobotidle}}
    	\State {$(S_R,End_H) \leftarrow\mathbf{reschedule}(T_H,S_R)$\label{algl:dsreschedule}}
    	\Else
    	\State {$End_R\leftarrow\mathbf{monitorR}(T_R)$ \label{algl:endr}}
    	\EndIf
    	\State $M_H\leftarrow \mathbf{read}_H()$, $M_R\leftarrow \mathbf{read}_R()$\label{algl:readmess}
    	\State {$(End_H,End_R,S_H,S_R)=$}
\item[]\hspace{1.5cm}{$\mathbf{communication}(M_H, M_R, S_H,S_R)$} \label{algl:dscommunication}%Unify the communication function
    	\If{$End_H$}
    	$T_H\leftarrow\mathbf{next} (T_H,S_H(l)$\label{algl:dsnextH}
    	\EndIf
    	\If{$End_R$}
    	$T_R\leftarrow\mathbf{next} (T_R,S_R(l))$\label{algl:dsnextR}
    	\EndIf
    	\EndWhile
    	\State{$l\leftarrow l+1$ \label{alg:dsnextlevel}}
    	\EndWhile
    	\State{$\mathbf{updateJQ()}$\label{alg:dsupdate}}
    \end{algorithmic}
\end{algorithm}	
	
	
The dynamic scheduler needs as an input the nominal tasks schedules $S_H$ and $S_R$ (Line~\ref{algl:dsrequire}). It immediately sets to false the two variables $End_R$ and $End_H$ that identify when the task currently associated to the robot and to the human have been concluded (Line~\ref{algl:dsinitializeends}) and it initializes the job at the first level (Line~\ref{algl:dsinitializelevel}). Subsequently, the algorithm checks if the two agents should execute at least one task in the first level and, if required, it assigns the first tasks of $S_R(l)$ and $S_H(l)$ to the human and to the robot (Line~\ref{algl:dsinitializetasksstart}-\ref{algl:dsinitializetasksend}). At this point, it starts two loops: one to iterate through the levels of the job (Line~\ref{algl:dswhilelevels}) and one to check when no more tasks for the robot and for the human are available in the current level (Line~\ref{algl:dswhiletasks}). Inside the second loop, the scheduler first checks if the robot has performed all its tasks in the level and it is waiting for the human to finish his task (Line~\ref{algl:dsrobotidle}). If the robot is in idle state, its list of tasks is adapted through the monitoring of the human's real execution time, in order to maximize the parallelism between the two agents (Line~\ref{algl:dsreschedule}).  In the other cases the algorithm checks if the robot has finished the assigned task (Line~\ref{algl:endr}). The function $\mathbf{monitoR}(T_R)$ is application dependent and it verifies (e.g. by a camera, by a timeout procedure) if the task $T_R$ has been successfully accomplished. If this is the case, the $\mathbf{monitorR}$ function returns a $true$ value, $false$ otherwise. The $\mathbf{monitorR}()$  function can be implemented using standard procedures, available for robotic applications (see e.g. \cite{pettersson2005}). If the robot cannot succeed to execute $T_R$ (e.g. though a timeout error), a $delegate$ message $M_R$ is communicated. Subsequently, all the messages generated by the human and the robot are considered for task swapping (Line~\ref{algl:dscommunication}). Finally, the algorithm checks if the task assigned to the human and to the robot are done and, if it is the case, assigns them the next task in the level (Lines~\ref{algl:dsnextH},~\ref{algl:dsnextR}). The function $\mathbf{next}(T,S(l))$ returns the task after $T$ in the same level $l$ of the Schedule $S$ and, if $T$ is the last task of the list, it returns $\emptyset$. When both $T_R$ and $T_H$ are empty, then the level is concluded and the job moves on to the next one (Line~\ref{alg:dsnextlevel}), restarting the loop until the last level is terminated. Finally, when all the tasks have been performed, the job quality parameters are updated through the function $\mathbf{updateJQ()}$ (Line~\ref{alg:dsupdate}) and used as input for the Task Assignment of the next job.
		
The rescheduling algorithm is represented in Alg.~\ref{alg:reschedule}.
\begin{algorithm}
	\caption{Reschedule()}
	\label{alg:reschedule}
	\begin{algorithmic}[1]
		\State \textbf{Require:} $T_H$, $S_R$ \label{algl:rsrequire}
		\State $t_{res}\leftarrow \mathbf{monitorH}(T_H)$\label{algl:rsmonitor}
		\If{$t_{res}>t_{Ri}$} \label{algl:rscheckresidualtime}
		\State $(pS_R,fS_R) \leftarrow \mathbf{split}(T_R,S_R)$\label{algl:rssplit}
		\State $fS_R^r \leftarrow\mathbf{fill}(fS_R,t_{res}-t_{Ri})$\label{algl:rsknap}
		\State $S_R \leftarrow\mathbf{concat}(pS_R. S_R^r,fS_R/fS_R^r)$\label{algl:rsconcat}
		\EndIf
		\State $End_H \leftarrow \mathbf{not} t_{res}$\label{algl:rsendH}
		\State $\mathbf{return} (S_R,End_H)$\label{algl:rsreturn}
	\end{algorithmic}
\end{algorithm}	
The algorithm requires as  input the tasks $T_H$ is currently assigned to the human and the current schedule $S_R$ of the tasks for the robot (Line~\ref{algl:rsrequire}). The activity of the human is monitored and the remaining time $t_{res}$ for the accomplishment of $T_H$ is estimated (Line~\ref{algl:rsmonitor}). The procedure \textbf{monitorH} can be implemented using several strategies available in the literature as, e.g., \cite{vo2014,maeda2017,maderna2019}. If $t_{res}$ is greater than the time necessary for the execution of some tasks in $S_R$, then these tasks may be executed in parallel with $T_H$ and, therefore, the rescheduling procedure starts (Line~\ref{algl:rscheckresidualtime}). First, the remaining schedule $S_R$ is split into two sub-lists: $pS_R$ contains all the robot assigned tasks in the actual level while $fS_R$ contains all the tasks of the next levels, which still need to be performed (Line~\ref{algl:rssplit}). Then, from $fS_R$, a sublist $S_R^r$ is generated (Line~\ref{algl:rsknap}). This sublist contains all the tasks that can be executed in the extra time available $t_{res}-t_{Ri}$ and whose precedences have already been executed. The list $S_R^r$ can be generated using any version of the well-known knapsack algorithm \cite{knapsack2000} or more simple, job dependent, search techniques. Finally the set of robot tasks of the level $S_R(l)$ is updated by  concatenating $pS_R$, with the list of the rescheduled tasks $fS_R^r$ (Line~\ref{algl:rsconcat}). After the rescheduling, the $End_H$ is set to $true$ if $T_H$ is over or to $false$ otherwise (Line~\ref{algl:rsendH}) and, finally, the new schedule $S_R$ and the $End_H$ variable are returned. 
		
During the execution of the job the human and the robot can generate messages in order to communicate to the Dynamic Scheduler the intention or need to swap their tasks. A detailed representation of this communication layout is shown in Fig.~\ref{fig:messages}.
\begin{figure}[t]
\vspace*{5pt}
	\centerline{\includegraphics[width=\columnwidth]{messages.png}}
	\caption{Communication Layout. The dotted lines indicate the ``reassign" message coming from the human and the consequent task scheduling. The dashed lines indicate the ``delegate" message coming from the human with the following scheduling to the robot. Finally, the brown lines indicate the ``delegate" message communicated by the robot.}
	\label{fig:messages}
\end{figure}
In particular, the message $M_R$ sent by the robot can be either empty or containing the value ``delegate $T_{R}$''  and it is generated by the \textbf{monitorR} function when the robot cannot succeed in executing the assigned task. The message $M_H$ can be either empty or it can assume two values: ``reassign $T_{reas}$'' or ``delegate $T_{del}$''. The first message is generated when the human decides to execute the task that the robot is executing (because, e.g., the robot is not doing the assigned work properly or in the best way). The second message is generated when the human decides to delegate some the the tasks in $S_H$ to the robot. This message has an argument, that specifies the task to be delegated. The human can enter the messages through a proper, job dependent, input interface. The messages generated by the human and by the robot are handled by Alg.~\ref{alg:communication}.
	
\begin{algorithm}
	\caption{Communication()}
	\label{alg:communication}
	\begin{algorithmic}[1]
		\State \textbf{Require:} $M_H$, $M_R$, $T_R$, $S_H$,$S_R$ \label{algl:corequire}
		\If{$M_H=reassign(T_{reas})$ } 
		\State $End_R\leftarrow true$\label{algl:coendr}
		\State $End_H\leftarrow true$\label{algl:coendh}
		\If{$T_{reas} = T_R$} \label{algl:cochecktreas}
			\State$S_R\leftarrow\mathbf{push}(T_{home},S_R)$\label{algl:copushhome1}
		\EndIf
		\State
		$S_R\leftarrow\mathbf{delete}(T_{reas},S_R)$\label{algl:codelete3}
		\State  $S_H\leftarrow\mathbf{push}(T_{reas},S_H)$\label{algl:copushRH}
		\ElsIf{$M_H=delegate(T_{del})$ \textbf{and} $\mathbf{exRobot}(T_{del})$}\label{algl:cocheckexrob}
		\State $S_H\leftarrow\mathbf{delete}(T_{del},S_H)$\label{algl:codelete1}
		\State   $S_R\leftarrow\mathbf{push}(T_{del},S_R)$\label{algl:copushdelR}
		\EndIf
		\If{$M_R=delegate(T_{R})$ \textbf{and} $\mathbf{exHuman}(T_R)$}\label{algl:cocheckexhum}
		\State $End_R\leftarrow true$\label{algl:coendr2}
		\State $S_R\leftarrow\mathbf{delete}(T_R,S_R)$\label{algl:codelete2}
		\State $S_R\leftarrow\mathbf{push}(T_{home},S_R)$\label{algl:copushhomeR}
		%  \State $End_H\leftarrow true$\label{algl:coendh2}
		\State   $S_R\leftarrow\mathbf{push}(T_R,S_H)$\label{algl:copushRH2}
		\EndIf
		\State $\mathbf{return}$ $End_H$, $End_R$, $S_H$, $S_R$\label{algl:coreturn}
	\end{algorithmic}
\end{algorithm}	
	
The algorithm requires the messages generated by human and robot $M_R$ and $M_H$ and the current schedules $S_R$ and $S_H$ and the task $T_R$ currently assigned to the robot (Line~\ref{algl:corequire}). The message $M_H$ is the first to be handled in order to give priority to the decisions taken by the operator. If the human decides to execute a task that was initially assigned to robot (i.e. $M_H = ``reassign$ $T_{reas}"$), both the end of the task variables are set to true. In this way, in Alg.~\ref{alg:dynamicscheduler}, the robot and the human will be assigned a new task (Lines~\ref{algl:coendr} and \ref{algl:coendh}). If the reassigned task is the one that the robot is executing (Line~\ref{algl:cochecktreas}), an homing task $T_{home}$ is put as the next task in the robot schedule (Line~\ref{algl:copushhome1}). The task $T_{reas}$ is then deleted from $S_R$ (Line~\ref{algl:codelete3}) while the task $T_R$ is pushed in the first position of the human schedule (Line~\ref{algl:copushRH}). In this way, the Alg.~\ref{alg:dynamicscheduler} will allocate $T_{home}$, that will send the robot to a safe home position, and $T_R$, the task the human has decided to execute, as the next tasks for the robot and the human. If the human decides to allocate a task $T_{del}\in S_H$ (i.e. $M_H =``delegate$ $T_{del}"$) and the task is executable by the robot (Line~\ref{algl:cocheckexrob}), then $T_{del}$ is deleted from $S_H$ (Line~\ref{algl:codelete1}) and transferred into the task schedule of the robot (Line~\ref{algl:copushdelR}). 
If the robot detects that it cannot fulfill the assigned task (i.e. $M_R=``delegate"$) and if the task it is trying to accomplish is executable by the human operator (Line~\ref{algl:cocheckexhum}), then the end of the task variable for the robot is set to $false$ to force Alg.~\ref{alg:dynamicscheduler} to allocate the next task to the robot. $T_R$ is deleted from the robot schedule $S_R$ (Line~\ref{algl:codelete2}) and inserted in the schedule of the human  (Line~\ref{algl:copushRH2}). Furthermore, an homing mission $T_{home}$ is added as the next task for the robot.
Finally the procedure returns the updated end of task variables and schedules (Line~\ref{algl:coreturn}).
The procedure \textbf{exRobot} and \textbf{exHuman} exploit prior information about the job and the tasks (e.g. the weights $w_{Ri}$ and $w_{Hi}$  in \eqref{eq:MILP}) to detect if a task can be executed by the robot or by the human.

Swapping the tasks between the human and the robot directly affects the job quality. Thus, it may happen that the final job quality indices do not respect the constraint imposed in the MILP problem \eqref{eq:MILP}. However, since the optimization problem requires as input the real job quality parameters, namely $K_{m,0}$, the possible work overload for the operator will be mitigated with subsequent task schedules. Another possible way to ensure the optimum of the job quality is the implementation of a function that checks if the task swapping will violate the constraints and, if required, prevents it. However the latter strategy is very conservative, as it does not take into account the possibility of correcting the job quality parameters in subsequent optimization problems. Furthermore, at the communication level, the job quality is treated as a soft constraint with respect to the need to swap a task (e.g. the robot failing a task is a more critical situation). For these reasons, in this paper it was decided not to investigate the latter solution.

% \apc{It is worth noting that the bottleneck of the Dynamic Scheduler is represented by the $\mathbf{fill()}$ function inside the $\mathbf{Reschedule()}$ algorithm (see Alg.~\ref{alg:reschedule}, Line \ref{algl:rssplit}). In its worst implementation this function has a complexity equal to $O(n+l)$, i.e. when analyzing every single element of the tuple . Since the number of tasks and levels in an industrial application is not that large, the algorithm is computationally cheap.}
It is worth noting that the Dynamic Scheduler is computationally cheap. The most heavy part is represented by the $\mathbf{fill()}$ function inside the $\mathbf{Reschedule()}$ algorithm (see Alg.~\ref{alg:reschedule}, Line \ref{algl:rssplit}). This function, in its worst implementation, has a linear complexity equal to $O(n+l)$, i.e. when analyzing every single element of the tuple with two \textit{for} cycles. Since the number of tasks and levels in an industrial application is not that large, the algorithm is reactive.

